HyperCam: Low-Power Onboard Computer Vision for IoT Cameras

We present HyperCam, an energy-efficient image classification pipeline that enables computer vision tasks onboard low-power IoT camera systems. HyperCam leverages hyperdimensional computing to perform training and inference efficiently on low-power microcontrollers. We implement a low-power wireless camera platform using off-the-shelf hardware and demonstrate that HyperCam can achieve an accuracy of 93.60%, 84.06%, 92.98%, and 72.79% for MNIST, Fashion-MNIST, Face Detection, and Face Identification tasks, respectively, while significantly outperforming other classifiers in resource efficiency. Specifically, it delivers inference latency of 0.08-0.27s while using 42.91-63.00KB flash memory and 22.25KB RAM at peak. Among other machine learning classifiers such as SVM, xgBoost, MicroNets, MobileNetV3, and MCUNetV3, HyperCam is the only classifier that achieves competitive accuracy while maintaining competitive memory footprint and inference latency that meets the resource requirements of low-power camera systems.

==> 3A-SystemDesign-Backup.tex <==
\section{\tool Design}

\tool processes computer vision tasks on the endpoint device (e.g., wireless IoT camera). When the camera captures an image, that image is converted into a hypervector, and the classifier determines its class based on the Hamming distance. Depending on the identified category, \tool can perform immediate actions such as displaying information on a monitor or unlocking a door. In addition, \tool can send the classification result to an IoT gateway via Bluetooth, allowing for remote monitoring and interaction. This approach of transmitting the classification data, as opposed to entire raw images, significantly minimizes communication overhead and mitigates the risk of transmission errors. At the gateway, data is pushed to the cloud for data storage and model improvements. Fig.\ref{fig:system_overview} shows the \tool system design and the following subsections describe the HDC-based classification model, the low-power hardware design, and the model's online learning approach in detail. \todo{vanilla encoding is the strawman approach, we propose hypercam that solves challenges}

\subsection{\tool{} Classifier Design}

The architecture for the \tool{} classifier, as shown in Fig.\ref{fig:system_overview}, has three major components: an image encoder, a training algorithm, and an inference algorithm. The image encoder translates raw image data to hypervectors that are then used by the training and inference algorithms. \tool{} uses the OnlineHD adaptive training algorithm to produce an item memory of hypervectors which are then stored on the microcontroller~\cite{onlinehd2021}. During execution, the microcontroller encodes each input frame into a hypervector with the image encoding algorithm and then performs HD classification by identifying the item memory hypervector with the smallest Hamming distance to the query hypervector. The microcontroller stores and uses \textit{hypervector codebooks} which are used to encode pixel and value information during the image encoding process, and the hypervector item memory to perform inference. 

A critical challenge with applying HD classifiers to image processing is managing performance and memory overheads associated with encoding image data as hypervectors 

\tool{} uses a novel hypervector image encoding 

identifying the hypervector in item memory 

During training, the OnlineHD adaptive training method is used to generate an item memory, which contains a hypervector for every class in the data \cite{onlinehd2021}. At inference, the encoded query hypervector is compared to every class hypervector based on a similarity metric, and the class with the minimum distance hypervector becomes the classification result. This model is used for face detection and identification that runs onboard the low-power wireless camera platform.

\begin{table*}[]
    \centering
    \begin{tabular}{|c|ccc|}
        \hline
         Encoding Method&  Vanilla &HyperCam &HyperCam + Caching\\
         \hline
         Num bundling& 
         $O(wh)$&$O(2^r)$ &1\\
         Codebook Num& $\textup{max}(w,h)$&$\left\lceil whd/n \right\rceil$ &$\left\lceil whd/n \right\rceil$ \\
        \hline
    \end{tabular}
    \caption{Comparison of different encoding methods \todo{work in prog}}
    \label{tab:encoding}
\end{table*}

\subsubsection{Vanilla Encoding}

The first step in the HDC-based classifier is to encode an image array into a hypervector. \tool's encoding scheme stems from the idea that each pixel contains two pieces of information: position and pixel intensity. Thus, \tool generates a codebook $H_1$ for pixel positions and a codebook $H_2$ for possible pixel values. $H_1$ is sufficient to represent different dimensions of an image (e.g., width, height, and depth) because permutations can be applied to differentiate dimensions as described in Section\ref{sec:permutation}. \tool works with grayscale images and therefore positional encoding uses column and width dimensions. Then, the hypervector of a pixel at $(i,j)$ of an image $I$  is encoded as the following,
\begin{equation}
    HV(I_{i,j}) = H_1(i) \odot \rho(H_1(j)) \odot H_2(I(i,j))
    \label{pixel-encoding}
\end{equation}
where $I(i,j)$ is the pixel value at position $(i,j)$. The hypervector of an image $I$ of width $w$ and height $h$ is the bundling of all pixel hypervectors,
\begin{equation}
    HV(I) = \sum_{i=1}^w\sum_{j=1}^h HV(I_{i,j}) \geq \frac{wh}{2}
    \label{image-encoding}
\end{equation}
As described in Section\ref{sec:bundling}, bundling is the majority vote of all pixel hypervectors, which is implemented as a summation of all pixel hypervectors and one element-wise value comparison. Despite the simplicity of its encoding scheme, this model encounters two significant hurdles in real-time processing. The encoding phase, as outlined in Eq. \ref{image-encoding}, necessitates $O(wh)$ bundling operations. As the size of the image increases, the encoding time rises proportionately. Given that the smallest acceptable image size for many vision tasks demands that $wh \geq 10^4$, the encoding step becomes the most time-consuming aspect of both model training and inference. Moreover, the storage requirement for this model is substantial. In this encoding scheme, $H_1$ is $\textup{max}(w, h, d) \times n$ array and $H_2$ is $2^r \times n$ where $r$ is the pixel resolution (e.g., eight for an 8-bit representation). These codebooks, along with the item memory generated from training, consume several megabytes of memory. They need to be stored on the device's permanent storage and transferred to device cache to facilitate fast access during encoding and prediction phases.

\subsubsection{\tool Encoding}
To reduce the computation overhead of bundling, \tool uses a modified encoding scheme based on sparse pixel encoding. Instead of using a dense binary hypervector, a sparse bipolar vector inspired from the count-sketch method is used as a basis hypervector representing a pixel position \cite{charikar2002finding}. In other words, each sparse vector has randomly selected $d$ non-zero elements, where each element is randomly set as $1$ or $-1$, with a probability of 0.5. Compared to the size of the hypervector $n$, $d \ll n$, in orders of magnitude.

Alg. \ref{alg:sparse} describes the encoding process based on these sparse hypervectors. First, a single pass is taken over the input image, during which the position hypervectors are summed according to their pixel values. This process is referred to as \textit{binning}, as it involves grouping and summing position hypervectors based on their corresponding pixel values. Next, the sum vectors are quantized to binary by mapping non-negative values to 1 and negative values to 0. These binary vectors can now use the standard BSC operators for binding and bundling. Each of these sum vectors, which have been binned by pixel values, are then bound with the corresponding value hypervector from the codebook. This results in $2^r$ hypervectors. These hypervectors are then bundled together, using weights equivalent to the number of pixels in each bin. The use of a sparse pixel representation significantly reduces the number of bundling operations from $whd$ to $2^r$. Moreover, since each hypervector contains only $d$ non-zero elements, the vector summation in the binning process computes $d$ integer elements instead of $n$.

% false positives? unbalanced class data
\todo{table to compare different encoding methods}

\begin{algorithm}
    \caption{Sparse hypervector encoding}
    \label{alg:sparse}
    \begin{algorithmic}
        \State Input: $I$ image
        \State $bins \gets 2^r \times n$ 0-valued matrix
        \State $counts \gets 2^r$ 0-valued vector
        \For{$i$ in $0..whd-1$}
            \State $v \gets I[i]$
            \State $bins[v] = bins[v] + posCodebook[i]$
        \EndFor
        \For{$v$ in $0..2^r$}
            \For{$i$ in $0..n$}
                \State $bins[v][i] = 1 ? bins[v][i] : 0$
            \EndFor
            \State bins[v] = bind($bins[v], valueCodebook[v]$)
        \EndFor
        \State bundle(bins)        
    \end{algorithmic}
\end{algorithm}

Further latency reduction can be achieved during inference where latency affects the service quality. \tool exploits the fact that for most face detection applications, the camera is in a static position and only parts of the image change at inference. A cache-based encoding scheme can reduce the processing latency by reducing the number of pixels to encode. At the camera startup, the background image $I_b$ and its encoded hypervector are stored in the hardware cache. The camera has an integrated motion sensor which is used as a trigger. Once triggered, the system captures an image $I$ and extracts its foreground $I_f$ by performing a differential operation with a threshold $t$.

\begin{equation}
    I_{f} = \textup{select}((I_{b} - I) \leq t)
\end{equation}

The encoder encodes this foreground as a hypervector and perform a weighted bundle with the cached background hypervector. The weight of the bundle is calculated by the proportion of the foreground to the image.

\begin{equation}
    \label{eq:diff}
    HV(I) = \frac{|I_f|}{|I|} HV(I_f) \oplus \left(1-\frac{|I_f|}{|I|}\right) HV(I_{b})
\end{equation}

Both $I_{b}$ and its hypervector $HV(I_{b})$ are stored in device cache. This encoding method reduces the number of bundling operations from $wh$ to 1, significantly reducing encoding time. More comparisons between encoding methods are shown in Table \ref{tab:encoding}.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{figs/diff-encoding.png}
%     \caption{Differential encoding method.}
%     \label{fig:diff-encoding}
% \end{figure}

\subsubsection{Training}
\tool uses the OnlineHD method for efficient and robust learning of the training data. A single pass of the training data is not sufficient to accurately extract the features. However, simply iterating over the data can lead to model saturation and forgetting. OnlineHD provides an effective single pass learning approach, where data is updated based on similarity to the existing model rather than naively accumulating data. The original OnlineHD model is implemented for a real-valued HDC model, not the BSC model. Therefore, the OnlineHD model is modified to handle BSC. In OnlineHD, model parameters are updated with a real-valued learning rate. To preserve the binary trait in the BSC encoding, the modified trainer hold two models during training, an unquantized and quantized version. The unquantized model is maintained for parameter updates. On the other hand, after each training iteration, a quantized model is derived from the unquantized model and is updated based on the Hamming distances between the training hypervectors and the quantized model. Alg. \ref{alg:onlinehd} describes this process.

\begin{algorithm}
    \caption{OnlineHD Trainer for BSC \todo{just the draft}}
    \label{alg:onlinehd}
    \begin{algorithmic}
        \Require $n \geq 0$
        \For{HV, label in trainHV}
            \State $dataset[label][i] += w * hv[i]$
        \EndFor
        \While{iteration < epoch}
            \State $distances \gets BSC.distance(HV, classHV)$
            \State $prediction \gets min(distances)$
        \EndWhile
    \end{algorithmic}
\end{algorithm}

\subsection{Model Optimization}
\tool's HDC-based classification model was trained offline on an Apple M1 Macbook Pro. Once the model training was complete, the model's codebook and item memory were exported as C arrays. These arrays are referenced as a header file on the embedded hardware. The critical requirement is that this header file must be small enough to fit the hardware's non-volatile memory. Additionally, at inference, it is important to optimize latency in order to maintain high service quality. Therefore, model optimizations to reduce both memory consumption and latency were implemented, as outlined below.

\subsubsection{Memory Optimization}

The memory footprint of the HDC model mostly comes from its codebook. In \tool, the encoding process requires two types of codebooks: positional codebook and pixel codebook. The positional codebook holds $\textup{max}(w,h)$ hypervectors, and the pixel codebook holds $2^r$ hypervectors, where $r$ is the pixel resolution. For example, for an image of size $160 \times 120$ represented as a byte, the positional codebook and the pixel codebook have $160$ and $256$ hypervectors, respectively, consuming megabytes of memory.

To reduce the size of the positional codebook, the encoding mechanism is modified to handle one-dimensional, flattened image data. Instead of pre-storing a unique basis hypervector for each position, a basis hypervector can be generated on-the-fly by applying permutations on a hypervector. For instance, if $v$ represents a basis hypervector, then for any given position $k$, the positional encoding for a pixel is denoted as $P_k(v)$. The pixel encoding at $I_k$ is,

\begin{equation}
    HV(I_k) = \rho_k(\vec{v}) \odot H(I(k))
    \label{1d-encoding}
\end{equation}

This method significantly reduces the memory demands from $\textup{max}(w,h)$ hypervectors to $\left\lceil whd/n \right\rceil$, where $n$ represents the length of the hypervector. For example, if f $n = 10000$, the codebook only holds 2 hypervectors.

Similarly, the pixel codebook can be dynamically generated during runtime. This codebook utilizes level encoding to ensure that numerically closer values are represented by similar hypervectors, while more distant values are represented by dissimilar hypervectors. The codebook initialization begins with an all-zero vector of length $n$ that represents a pixel value of zero. With each incremental value, the initial $n/2^r$ zero-valued bits in the vector are toggled to one. This approach to computing the pixel codebook does not add extra computational steps to the encoding process since it can be seamlessly integrated into the binding operation, which already iterates over the $n$ bits of the vector. As illustrated in Alg. \ref{alg:pixgen}, for a given value $v$, the first $v$ segments of $n/2^r$ bits are set to one, prompting the binding operation to invert the corresponding pixel values. The remaining segments, which retain their zero value, do not affect the outcome of this operation.

\begin{algorithm}
    \caption{Binding operation while generating pixel codebook on-the-fly}
    \label{alg:pixgen}
    \begin{algorithmic}
        \State $i = 0$
        \While{$i < v \cdot n/2^r$}
            \State $result[i] = pixel[i] \wedge 1$
            \State $i = i+ 1$
        \EndWhile
        \While{$i < n$}
            \State $result[i] = pixel[i]$
            \State $i = i+1$
        \EndWhile
    \end{algorithmic}
\end{algorithm}

\subsubsection{Latency Optimization}

To reduce the computation load, the binary hypervectors were packed into 16 and 32-bit data types. The ARM Cortex M-33 processor can use byte-level instructions to manipulate data, instead of bit-by-bit. In the BSC model, both the binding and permutation can handle byte-level data without overhead. For example, byte-level XOR works the same as the bit-level XOR. Byte-level permutation is to simply shift 8 more bits than bit-level permutation. However, transforming a bit-level bundling operation to byte-level requires huge overhead. While bit-level bundling is implemented as a summation of all bits in the same index, bytes cannot be summed in the same way because the summation results would ignore carries. Thus, every bit has to be unpacked and individually counted. This bit packing and unpacking process can be a bottleneck in the encoding process. We further experiment with bit packing based encoding in the Experiments section.

The smallest data type in the ARM Cortex M-33 processor is a byte. Thus, without bit packing, bits are stored in a byte array. This can cause memory overhead (\todo{tell why this is not the problem}), but we can now use vector operations to compute binding, bundling, and permutation.  We accelerate vector computation by using SIMD (Single Instruction, Multiple Data) operations such as QADD and QMULTIPLY to accelerate n-size vector computations. We also integrate the CMSIS (Cortex Microcontroller Software Interface Standard) DSP (Digital Signal Processing) library to use ARM native vector operations such as vector XOR. This approach has effectively halved the processing time.

Finally, the permutation operation is implemented  through array repeat. Instead of permuting the entire array in-place, the array size is doubled and the contents are repeated such that permutation can be implemented by modifying the indices. This approach reduces number of operations at every step of pixel iteration to be one instead of $N$.

% \subsection{Online Learning}

% One of the key features of an end-to-end system with a data-driven classifier is its ability to store, analyze, and utilize deployment data to refine the model. This is crucial because the deployment data might greatly vary from the training data distributions, with unseen categories of data potentially appearing. The system can adapt to these changes through online learning, or incremental learning, which involves integrating new data streams during deployment. \tool{} uses two strategies for online learning: one is entirely local, updating the \tool{}'s HDC-based model parameters on-device; the other leverages cloud support.

% \subsubsection{onboard Checkpointing}
% In HDC, the model is updated by combining the current class hypervector with the new data's encoded hypervector using a bundling operation. A major challenge with online learning is the risk of the model forgetting past information if updated too frequently with new data. To address this, a checkpointing strategy is introduced. This approach involves accumulating the hypervectors from several data instances into checkpoints, which are then integrated with the model's existing item memory. These checkpoints are saved in non-volatile memory, with each representing the collective hypervector of 1000 instances. To avoid rapid memory loss, at least 10 checkpoints are kept at any time. Furthermore, a counter is used to keep track of the created checkpoints, used in a weighted bundling process that ensures a balanced update.

% \subsubsection{Cloud Support}
% There are a few scenarios where \tool could benefit from cloud support, where less constraints are put on compute power and storage. \textbf{[provide example]}. Instead of solely relying on onboard computing, \tool can transmit the stored checkpoints (\textbf{size? few kB?}) to synchronize the local classifier with its cloud counterpart. The checkpoints, along with all past data and original train data are archived in the cloud and can accurately refine the classifier. When the model updates are significant, such as when new classes are added, the gateway send the new model memory to IoT camera to reflect the changes. 

% In instances where the HDC classifier outputs a low confident result, the hypervector of the input image is transmitted to the cloud. That image is flagged for manual review and annotation so that the model can learn from the corner cases. The choice of transmitting the hypervector instead of the raw image is to preserve communication resources.  A hypervector, composed of $n$ bits, is typically more compact than the conventional pixel representation of $wh$ bytes. 

% However, the challenge lies in the cloud's ability to accurately decode these hypervectors. Hypervector decoding relies on a distance metric within HDC encoding. For every position, every possible pixel hypervector is individually encoded to the position hypervector, creating $2^r$ candidate hypervectors. The candidate hypervector with the lowest Hamming distance to the query hypervector signifies that the pixel value used in the candidate is the decoded value. The process is lossy, but an average of X\% of the transmitted image were recovered.


==> Revision-Summary.tex <==
\section*{Revision Summary}

\noindent This work is submitted as part of the Revise and Resubmit in the Mobicom Winter 2024 cycle. Below are the revision items reviewers requested to be addressed:

\begin{itemize}
    \item[(1)] Add the following approaches to the baselines for comparison: (i) TinyML model MCUNet-Vx, (ii) lightweight machine learning methods including xgboost trees and SVM, (iii) compressed MobileNet and MicroNet by applying common quantization/pruning techniques.
    \item[(2)] Add at least two more datasets as the benchmarks to compare with baselines to show the generalizability of the approach.
    \item[(3)] Add a discussion on how the proposed approach could generalize to other microcontroller platforms.
\end{itemize}

\vspace{0.3cm}
\noindent Based on these suggestions, below are the major changes of this work.

\vspace{0.5cm}
\subsection*{Evaluation}

The reviewers have requested to add more baselines and benchmark datasets for comparison. We have added 7 more baseline classifiers, which include HD classifiers (Vanilla HDC, OnlineHD, Rewrite 2), lightweight ML models (SVM, xgBoost), and neural networks (MCUNetV3 in small and large sizes). Each baseline classifier is described in-depth in Section 6.1.2. Furthermore, we have added 2 more benchmark datasets, including MNIST and Fashion-MNIST datasets. These 2 datasets are widely used to evaluate machine learning classifiers. More difficult benchmark datasets such as ImageNet are not shown because edge machine learning models altogether don't perform well due to the task's difficulty and does not serve as a good benchmark. Section 6.1.1 describes the added datasets in-depth.\\

\noindent Additionally, addressing reviewer A's comments, we added peak RAM footprint as one of our classifier evaluation metrics. Section 6.1.3 describes the changes.\\

\noindent All new results from the added classifiers, datasets, and metrics are shown in Table 2 and explained in Section 6.2.
\vspace{0.5cm}
\subsection*{Other Microcontroller Platforms}

We talk about our tool's generalizability to other microcontroller platforms in Section 8. In summary, our tool does not require additional libraries and engines such as TensorFlow Lite Micro and CMSIS-NN or specialized hardware such as Neural Processing Units and Floating Point Units. Our tool only uses integer numbers (more specifically, bits) and harware-native bit operations such as addition and bit flips. Therefore, out tool is easily ported to any microcontroller by simply copying the provided C code, which includes the encoding and inference operations, and a header file, which includes a few binary arrays that represent the model weight. The only requirement is that the microcontroller must have a flash memory of at least 60 kilobytes and an active memory of at least 20 kilobytes.

\vspace{0.5cm}
\subsection*{Minor Revisions}

\begin{enumerate}
    \item Numerical change in Figure 7 to address the comment of Reviewer A.
    \item Equation change in Section 4.2.1 where $p^i$ was changed to $p^j$. This addresses the comment of Reviewer D.
    \item Dataset description in Section 5.2 to explain how many images and classes are in the collected dataset. This addresses the comment of Reviewer E.
\end{enumerate}

% \begin{itemize}
    % \item[(1)] Addition of baseline classifiers described in Section 6.1.2, which includes HD classifiers (Vanilla HDC, OnlineHD, Rewrite 2), lightweight ML models (SVM, xgBoost), and neural networks (MCUNet V3 in small and large sizes). Table 2 and Section 6.2 are updated to show new results and explain them along with previous results.
    % \item[(2)] Addition of benchmark datasets described in Section 6.1.1, which includes MNIST and Fashion-MNIST datasets. Table 2 and Section 6.2 are updated to show new results and explain them along with previous results.
    % \item[(3)] Discussion of generalizability of our method in Section 8.
    % \item[(1)] Numerical change in Figure 7 to address comments of Reviewer A.
    % \item[(5)] Addition of classifier evaluation metric, which now includes peak RAM usage, described in Section 6.1.2. Table 2 is updated accordingly.
% \end{itemize}

\vspace{0.5cm}
\subsection*{Marked-Up Manuscript}
\noindent A marked-up manuscript, where changes are \textcolor{blue}{highlighted}, is included below.
